Adversarial random forests for density estimation and generative modeling

We propose methods for density estimation and data synthesis using a novel form of unsupervised random forests. Inspired by generative adversarial networks, we implement a recursive procedure in which trees gradually learn structural properties of the data through alternating rounds of generation and discrimination. The method is provably consistent under minimal assumptions. Unlike classic tree-based alternatives, our approach provides smooth (un)conditional densities and allows for fully synthetic data generation. We achieve comparable or superior performance to state-of-the-art probabilistic circuits and deep learning models on various tabular data benchmarks while executing about two orders of magnitude faster on average. An accompanying $\texttt{R}$ package, $\texttt{arf}$, is available on $\texttt{CRAN}$.

==> AISTATS/app_exp.tex <==
Our experiments do not include any personal data, as defined in Article 4(1) of the European Union's General Data Protection Regulation. All data are either simulated or from publicly available resources. 
%such as the University of California Irvine Machine Learning repository \citep{Dua2019}.
We performed all experiments on a dedicated 64-bit Linux platform running Ubuntu 20.04 with an AMD Ryzen Threadripper 3960X (24 cores, 48 threads) CPU, 256 gigabyte RAM and two NVIDIA Titan RTX GPUs. We used $\texttt{R}$ version 4.1.2 and Python version 3.7.12. Further details on the environment setup are provided in the supplemental code. 

\subsection{Simulations}
The $\texttt{cassini}$, $\texttt{shapes}$, and $\texttt{smiley}$ simulations are all available in the $\texttt{mlbench}$ $\texttt{R}$ package; the $\texttt{twomoons}$ problem is available in the $\texttt{fdm2id}$ $\texttt{R}$ package. Default parameters were used throughout, with fixed sample size $n=2000$. 

\subsection{Twenty Datasets}\label{sec:appx_pc}

The Twenty Datasets benchmark was originally proposed by \citet{Davis_2021}. A conventional training/validation/test split is widely used in the PC literature. Because our method does not include any hyperparameter search, we combine training and validation sets into a single training set. We downloaded the data from \url{https://github.com/joshuacnf/Probabilistic-Generating-Circuits/tree/main/data} and include the directory in our project GitHub repository for completeness. 
All datasets are Boolean, with sample size and dimensionality given in Table \ref{tab:20datasets}.

\begin{table}[htbp]
\scriptsize
\centering
\caption{Summary of datasets included in the Twenty Datasets benchmark.}
\label{tab:20datasets}
\begin{tabular}{lrrrr}
\toprule
Dataset   & Train  & Validation & Test  & Dimensions \\ 
\midrule
\texttt{nltcs}     & 16181  & 2157       & 3236  & 16             \\
\texttt{msnbc}     & 291326 & 38843      & 58265 & 17             \\
\texttt{kdd}       & 180092 & 19907      & 34955 & 64             \\
\texttt{plants}    & 17412  & 2321       & 3482  & 69             \\
\texttt{audio}     & 15000  & 2000       & 3000  & 100            \\
\texttt{jester}    & 9000   & 1000       & 4116  & 100            \\
\texttt{netflix}   & 15000  & 2000       & 3000  & 100            \\
\texttt{accidents} & 12758  & 1700       & 2551  & 111            \\
\texttt{retail}    & 22041  & 2938       & 4408  & 135            \\
\texttt{pumsb}     & 12262  & 1635       & 2452  & 163            \\
\texttt{dna}       & 1600   & 400        & 1186  & 180            \\
\texttt{kosarek}   & 33375  & 4450       & 6675  & 190            \\
\texttt{msweb}     & 29441  & 3270       & 5000  & 294            \\
\texttt{book}      & 8700   & 1159       & 1739  & 500            \\
\texttt{movie}     & 4524   & 1002       & 591   & 500            \\
\texttt{webkb}     & 2803   & 558        & 838   & 839            \\
\texttt{reuters}   & 6532   & 1028       & 1540  & 889            \\
\texttt{20ng}      & 11293  & 3764       & 3764  & 910            \\
\texttt{bbc}       & 1670   & 225        & 330   & 1058           \\
\texttt{ad}        & 2461   & 327        & 491   & 1556           \\
\bottomrule
\end{tabular}
\end{table}

Results for competitors are reported in the cited papers:
\begin{itemize}[noitemsep]
    \item Einsum networks \citep{peharz2020}
    \item Random sum-product networks \citep{ratspn}
    \item Probabilistic generating circuits \citep{zhang2021}
    \item Strudel \citep{dang2022}
    \item Continuous mixtures of Chow-Liu trees \citep{correia2022}.
\end{itemize}

\subsection{Tabular GANs}\label{sec:appx_gan}
For benchmarking generative models on real-world data, we use the benchmarking pipeline proposed by \citet{Xu2019}. In detail, the workflow is as follows:
\begin{enumerate}
    \item Load classification datasets used in \citet{Xu2019}, namely $\texttt{adult}$, $\texttt{census}$, $\texttt{credit}$, $\texttt{covertype}$, $\texttt{intrusion}$, $\texttt{mnist12}$, and $\texttt{mnist28}$. Note that the type of prediction task does not affect the process of synthetic data generation, so we omit the single regression example ($\texttt{news}$) for greater consistency. 
    \item Split the data into training and test sets (see Table~\ref{benchmark_details} for details).
    \item Train the generative models $\textsc{Forge}$ (number of trees $=10$, minimum node size $=5$),  $\textsc{ctgan}$\footnote{\url{https://sdv.dev/SDV/api_reference/tabular/ctgan.html}. MIT License.} (batch size $= 500$, epochs $=300$), $\textsc{tvae}$\footnote{\url{https://sdv.dev/SDV/api_reference/tabular/tvae.html}. MIT License.} (batch size $= 500$, epochs $=300$), $\textsc{ctab-gan+}$\footnote{\url{https://github.com/Team-TUD/CTAB-GAN-Plus}} (batch size $= 500$, epochs $= 150$), $\textsc{it-gan}$\footnote{\url{https://github.com/leejaehoon2016/ITGAN}. Samsung SDS Public License V1.0.} (batch size $= 2000$, epochs $= 300$) and $\textsc{rcc-gan}$\footnote{\url{https://github.com/EsmaeilpourMohammad/RccGAN}} (batch size $= 500$, epochs $= 300$).
    \item Generate a synthetic dataset of the same size as the training set using each of the generative models trained in step (3), measuring the wall time needed to execute this task.
    \item Train a set of supervised learning algorithms (see Table~\ref{benchmark_details} for details): (a) on the real training data set (i.e., the \textit{Oracle}); and (b) on the synthetic training datasets generated by $\textsc{Forge}$,  $\textsc{ctgan}$, $\textsc{tvae}$, $\textsc{ctab-gan+}$ and $\textsc{rcc-gan}$.
    \item Evaluate the performance of the learning algorithms from step (5) on the test set.
    \item For each dataset, average performance metrics (accuracy, F1-scores) across learners. We report F1-scores for the positive class, e.g. `>50k' for \texttt{adult}, `+50000' for \texttt{census} and `1' for \texttt{credit}.
\end{enumerate}



\begin{table}[htbp]
\scriptsize
\centering
\caption{Benchmark Setup. Supervised learning algorithms for prediction: (A) Adaboost, estimators = 50 , (B) Decision Tree, tree depth for binary/multiclass target = 15/30, (C) Logistic Regression, (D) MLP, hidden layers for binary/multiclass target = 50/100}
\label{benchmark_details}
\begin{tabular}{llll}
\toprule
Dataset & Train/Test & Learner & Link to dataset\\ \midrule
\texttt{adult} \citep{Dua2019} & 23k/10k & A,B,C,D &\url{http://archive.ics.uci.edu/ml/datasets/adult}\\ 
\texttt{census} \citep{Dua2019} & 200k/100k & A,B,D &\url{https://archive.ics.uci.edu/ml/datasets/census+income} \\
\texttt{covertype} \citep{covertype} & 481k/100k & A,D &\url{https://archive.ics.uci.edu/ml/datasets/covertype} \\
\texttt{credit} \citep{credit} & 264k/20k & A,B,D &\url{https://www.kaggle.com/mlg-ulb/creditcardfraud}\\
\texttt{intrusion} \citep{Dua2019} & 394k/100k & A,D &\url{http://archive.ics.uci.edu/ml/datasets/kdd+cup+1999+data}\\
\texttt{mnist12} \citep{mnist} & 60k/10k & A,D & \url{http://yann.lecun.com/exdb/mnist/index.html}\\
\texttt{mnist28} \citep{mnist} & 60k/10k & A,D & \url{http://yann.lecun.com/exdb/mnist/index.html}\\
\bottomrule 
\end{tabular}\end{table} 

\subsection{Run Time}\label{app:runtime}

In order to evaluate the run time efficiency of $\textsc{Forge}$, we chose to focus on the smallest dataset of the benchmark study in Sect.~\ref{sec:benchmark}, namely \texttt{adult}. We \textbf{(A)} drew stratified subsamples and \textbf{(B)} drew covariate subsets. For step \textbf{(B)}, the target variable is always included. We select an equal number of continuous/categorical covariates when possible and use all $n = 32,561$ instances. Results in terms of processing time are visualized in Fig.~\ref{fig:process_time}. 
%Note that we use default parameters for $\textsc{ctgan}$ and $\textsc{tvae}$, which include automated parallelization over all available cores.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.85\textwidth]{process_time2.pdf}
  \caption{Complexity curves. \textbf{(A)}: Processing time as a function of sample size, using stratified subsamples of the \texttt{adult} dataset. \textbf{(B)}: Processing time as a function of dimensionality, using random features from the \texttt{adult} dataset.}
  \label{fig:process_time}
\end{figure} 

\subsection{Image Data}\label{sec:mnist}
We include results on the $\texttt{mnist12}$ and $\texttt{mnist28}$ datasets here, both included in the original \citet{Xu2019} pipeline. Benchmarking against $\textsc{ctgan}$ and $\textsc{tvae}$ (other methods proved too slow to test), we find that $\textsc{Forge}$ outperforms both competitors in accuracy, F1-score, and speed (see Table \ref{tbl:mnist}).

\begin{table}[htbp]
\scriptsize
\centering
\caption{Performance on $\texttt{mnist}$ datasets from the \citet{Xu2019} benchmark for $\textsc{ctgan}$ and $\textsc{tvae}$ vs. $\textsc{Forge}$ We report average results across five replicates $\pm$ the associated standard error. Winning results in bold.}
\label{tbl:mnist}
\begin{tabular}{llccr}
  \toprule
Dataset & Model & Accuracy $\pm$ SE  & F1 $\pm$ SE & Time (sec) \\ 
  \midrule
  \texttt{mnist12} & \textit{Oracle} & \textit{0.892 $\pm$ 0.003} & \textit{0.891 $\pm$ 0.003} &  \\ 
   classes = 10 & $\textsc{Forge}$ & \textbf{0.799} $\pm$ 0.007 & \textbf{0.795} $\pm$ 0.007 & \textbf{32.3} \\ 
   $n $ = 70,000 & $\textsc{ctgan}$ & 0.172 $\pm$ 0.032 & 0.138 $\pm$ 0.032 & 2737.4 \\ 
   $d$ = 144 & $\textsc{tvae}$ & 0.763 $\pm$ 0.002 & 0.761 $\pm$ 0.002 & 1143.8 \\ \midrule
  \texttt{mnist28} & \textit{Oracle} & \textit{0.918 $\pm$ 0.002} & \textit{0.917 $\pm$ 0.002} & \\ 
   classes = 10 & $\textsc{Forge}$ & \textbf{0.729} $\pm$ 0.008 & \textbf{0.723} $\pm$ 0.008 & \textbf{169.5} \\ 
   $n $ = 70,000 & $\textsc{ctgan}$ & 0.197 $\pm$ 0.051 & 0.167 $\pm$ 0.051 & 14415.4 \\ 
   $d$ = 784 & $\textsc{tvae}$ & 0.698 $\pm$ 0.016 & 0.697 $\pm$ 0.016 & 5056.0 \\ 
   \bottomrule
\end{tabular}
\end{table}

However, since MNIST is not a tabular data problem, perhaps a more relevant comparison would be against convolutional networks specifically designed for image data. We train a conditional GAN with convolutional layers \citep{cgan2014} and find that the resulting $\texttt{cGAN}$ clearly outperforms $\textsc{Forge}$ (see Fig. \ref{fig:mnist28}). This result is expected, given that our method is not optimized for image data. It also illustrates a limitation of our approach, which excels in speed and flexibility but is no match for deep learning methods on structured datasets.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{mnist28.png}
  \caption{Results from $\texttt{mnist28}$ experiment. \textbf{(A)}: Original samples. \textbf{(B)}: Samples generated by cGAN. \textbf{(C)}: Samples generated by $\textsc{Forge}$.}
  \label{fig:mnist28}
\end{figure} 


==> AISTATS/app_proofs.tex <==
\subsection{Proof of Thm.~\ref{thm:conv}}\label{proof:conv}
To secure the result, we must show that (a) the discriminator reliably converges on the Bayes risk at each iteration $t$; and (b) the generator's sampling strategy drives original and synthetic data closer together, ultimately taking the Bayes risk to $1/2$ as $n, t \rightarrow \infty$. (For the purposes of this proof, we set the tolerance parameter $\delta$ to $0$.)

Take (a) first. This amounts to a consistency requirement for RFs.
The consistency of RF classifiers has been demonstrated under various assumptions about splitting rules and stopping criteria \citep{breiman2004, biau_consistency, biau2010, gao2020}, but these results generally require trees to be grown to purity or even completion (i.e., $n^\ell_b = 1$ for all $\ell, b$). However, this would turn the generator's sampling strategy into a simple copy-paste operation and make intra-leaf density estimation impossible. We therefore follow \citet{Malley2012} in observing that regression procedures constitute probability machines, since $P(Y=1|\mathbf{x}) = \mathbb{E}[Y|\mathbf{x}]$ for $Y \in \{0, 1\}$. 

For simplicity, we focus on the single tree case, as the consistency of the ensemble follows from the consistency of the base method \citep{biau_consistency}. We define $\eta^{(t)}(\mathbf{x}) := P(Y=1|\mathbf{x}, t)$ as the target function for fixed $t$. Let $f_n^{(t)}(\mathbf{x})$ be a tree trained according to (A1)-(A3) on a sample of size $n$ at iteration $t$. Since $L_2$-consistency entails classifier consistency using the soft labeling approach of (A3).(vi), our goal in this section is to show that, for all $t \in \mathbb{N}$, we have:
\begin{align*}
    \lim_{n \rightarrow \infty} \mathbb{E} \Big[ \big(f_n^{(t)}(\mathbf{x}) - \eta^{(t)}(\mathbf{x})\big)^2 \Big] = 0.
\end{align*}
Consistency for RF regression has been established for several variants of the algorithm, occasionally under some constraints on the data generating process \citep{genuer2012, Scornet2015, wager_walther, Biau2016}. Recent work in this area has tended to focus on asymptotic normality \citep{mentch2016, Wager2018, Athey2019, Peng2022}, which requires additional assumptions. These often include an upper bound on leaf sample size, which would complicate our analysis in Thm.~\ref{thm:cons}. To avoid unnecessary difficulties, we borrow selectively from \citet{Meinshausen2006}, \citet{biau_analysis}, \citet{denil2014}, \citet{scornet2016_asymptotics}, and \citet{Wager2018}, striking a delicate balance between theoretical parsimony and fidelity to the classic RF algorithm.\footnote{Several authors have conjectured that RF consistency may not require honesty (A3).(i) or subsampling (A3).(ii) after all. Empirical performance certainly seems unencumbered by these requirements. However, both come with major theoretical advantages---the former by making predictions conditionally independent of the training data while preserving some form of adaptive splits, the latter by avoiding thorny issues arising from duplicated samples when bootstrapping. See \citet[Rmk.~8]{biau_analysis}, \citet[Appx.~B]{Wager2018}, and \citet{tang2018} for a discussion.} 

For full details, we refer readers to the original texts. The main point to recognize is that, under assumptions (A1)-(A3), RFs satisfy the conditions of Stone's theorem \citep{stone1977}, which guarantees the universal consistency of a large family of local averaging methods. 
\citet[Thm.~6.1]{devroye1996} and \citet[Thm.~4.2]{gyorfi2002} show that partitioning estimators such as decision trees qualify provided that (1) $\text{diam}(\mathcal{X}_\ell) \rightarrow_p 0$ and (2) $n_\ell \rightarrow_p \infty$ for all $\ell$ as $n \rightarrow \infty$, effectively creating leaves of infinite density. The former is derived by \citet[Lemma 2]{Meinshausen2006} under (A3).(iii) and (A3).(iv); the latter follows trivially from (A3).(v). Thus RF discriminators weakly converge on the Bayes risk in the large sample limit, completing part (a) of the proof.

Desideratum (b) effectively says that original and synthetic data become indistinguishable as $n$ and $t$ increase. 
Recall that at $t=0$, we generate synthetic data $\tilde{\mathbf{X}}^{(0)} \sim \prod_{j=1}^d P(X_j)$, which becomes input to the discriminator $f^{(0)}_n$. Let $\bm{\theta}^{(0)}$ denote the resulting splits once the discriminator has converged.
In subsequent rounds, synthetic data are sampled according to $\tilde{\mathbf{X}}^{(t+1)} \sim \prod_{j=1}^d P(X_j|\theta_\ell^{(t)})P(\theta_\ell^{(t)})$. (The consistency of coverage estimates is treated separately in Appx.~\ref{proof:l2}.)
We proceed to train a new discriminator and repeat the process. 

Let $P^*$ be the target distribution and $P^{(t)}$ the synthetic distribution at round $t$. For all $t \geq 1$, the input data to the discriminator $f^{(t)}_n$ is the dataset $\mathcal{D}_n^{(t)} \sim 0.5P^* + 0.5P^{(t-1)}$. Our goal in this section is to show that, as $n, t \rightarrow \infty$:
\begin{align*}
    \sup_{\mathbf{x} \in \mathcal{D}_n^{(t)}} |\eta^{(t)}(\mathbf{x}) - 1/2| \rightarrow_p 0.
\end{align*}

An apparent challenge to our recursive strategy for generating synthetic data is posed by self-similar distributions, in which dependencies replicate at ever finer resolutions, as in some fractal equations \citep{mandelbrot1982}. For instance, let $g$ be the Weierstrass function \citep{Weierstrass1895}, and say that $X_2 = g(X_1)$. Then the generative model will tend to produce off-manifold data at each iteration $t$, no matter how small $\text{vol}(\mathcal{X}_\ell)$ becomes. However, this only shows that convergence can fail for finite $t$.
Since the discriminator is consistent, it will accurately identify synthetic points in round $t+1$, pruning the space still further.

Let $[L^{(t)}]$ be the leaves of the discriminator $f^{(t)}_n$, and define the maximum leaf diameter $m_t := \max_{\ell \in [L^{(t)}]} \text{diam}(\mathcal{X}_\ell)$.We say that two samples are \textit{neighbors} in $f_n^{(t)}$ if the model places them in the same leaf.
We show that, as $n, t \rightarrow \infty$, conditional probabilities for neighboring samples converge---including, crucially, original and synthetic counterparts. Our Lipschitz condition (A2) states that for all $\mathbf{x}, \mathbf{x}'$, we have:
\begin{align*}
    |\eta^{(t)}(\mathbf{x}) - \eta^{(t)}(\mathbf{x}')| \leq c_t ~\lVert \mathbf{x} - \mathbf{x}' \rVert_2,
\end{align*}
where $c_t$ denotes the Lipschitz constant at round $t$. 
Suppose that $\mathbf{x}$ and $\mathbf{x}'$ are neighbors. 
Then we can replace the second factor on the rhs with $m_t$, since the $L_2$ distance between neighbors cannot exceed the maximum leaf diameter at round $t$. \citet{Meinshausen2006}'s aforementioned Lemma 2 ensures that this value goes to zero in probability as rounds increase. This could in principle be offset by a sufficient increase in $c_t$ over training rounds, but the second condition of (A2) prevents this, imposing the constraint that $c_t = o(m_t^{-1})$. Thus, for observations in the same leaf, $c_tm_t \rightarrow_p 0$ as $t \rightarrow \infty$. 
Because original and synthetic samples are equinumerous in all leaves following the generative step, each original sample has a synthetic counterpart to which it is arbitrarily close in $L_2$ space as $t$ grows large. Since no feature values are sufficient to distinguish between the two classes in any region, all conditional probabilities go to 1/2, and Bayes risk therefore also converges to 1/2 in probability. This concludes the proof. 

\begin{comment}
%Observe that the $L_2$ distance between any $\mathbf{x}, \tilde{\mathbf{x}}^{(t)}$ generated from the same leaf $\ell$ is at most $\text{diam}(\mathcal{X}_\ell)$. Because our stopping rule implies $\lim_{t \rightarrow \infty} m(t)=0$, original and synthetic samples become arbitrarily close as rounds increase. By the continuity assumption (A2), this means the gap between $P(Y=1|\mathbf{x})$ and $P(Y=1|\tilde{\mathbf{x}}^{(t)})$ also goes to zero as $t$ grows. (The extra condition on Lipschitz constants ensures that the rhs of the Lipschitz inequality decreases with $t$.) Thus the two classes cannot be reliably distinguished and Bayes risk converges to 1/2. 

%In the asymptotic regime, we need some stopping criterion to trigger potential recursion, or else we are indefinitely stuck on $t=0$. 
%Let $\text{diam}(\ell)$ denote the diameter of leaf $\ell$, i.e. the length of the longest segment contained in $\mathcal{X}_\ell$. 
%\citet[Lemma 2]{Meinshausen2006} shows that under the regularity conditions of (A3), $\text{diam}(\mathcal{X}_\ell) \rightarrow_{p} 0$ for all $\ell$ as $n \rightarrow \infty$. 
%For the purposes of this proof, we consider a modified version of Alg. \ref{alg:arf} in which training rounds terminate when this value falls below a threshold that decreases with $t$. That is, for all $t \in \mathbb{N}$ and some $v > 0$, we grow $f^{(t)}_n$ until $m(t) \leq v/(t+1)$. 

 
%We then sample leaves according to their coverage $\ell \sim q(\theta_\ell_0)$, and generate new data $\tilde{\mathbf{X}}^{(1)} \sim \prod_{j=1}^d P(X_j|\theta_\ell_0)$, which in turn becomes input to the discriminator $f^{(1)}$. This sampling strategy tends to down-weight low-density regions and concentrate in high-density regions. (The consistency of coverage estimates is treated separately in Appx.~\ref{proof:l2}.) Leaves with relatively little real data are unlikely to be the source of synthetic samples in subsequent rounds, where new observations are drawn instead from leaves that overlap more closely with the true data manifold.
%The only way this strategy could err in the asymptotic regime is if the target distribution were self-similar, with dependencies replicating at ever finer resolutions, as in some fractal equations \citep{mandelbrot1982}. But this would violate (A2), which states that no feature is a deterministic function of the others. A noisy fractal raises no fundamental challenge. Eventually the maximum leaf diameter becomes smaller than the residual variance. Now we have an infinitesimally small bounding box in which to sample synthetic data. Since these points are arbitrarily close to their original counterparts from the same leaf, the two classes cannot be reliably distinguished and Bayes risk converges to $1/2$.  

%As the synthetic data draws closer to the original with each passing round, the maximum leaf diameter shrinks, creating leaves of increasing density. This results in 



Let $\mathcal{D}_n^{(t)} = \{\mathbf{x}_i, 1\}_{i=1}^n \cup \{\tilde{\mathbf{x}}_i, 0\}_{i=1}^n$ be the complete dataset of original and synthetic samples generated at round $t$, which are subsequently used as input to model $f_n^{(t)}$. We denote the true labels for this dataset as $Y_n^{(t)}$.
Let $\hat{Y}_n^{(t)}$ be a random Boolean variable whose $i$th instance is $\mathbb{I}[f_n^{(t)}(\mathbf{x}_i) > 1/2]$, i.e. the hard labels associated with a given model. Our goal in this section is to show that, as $n, t \rightarrow \infty$:
\begin{align*}
    \mathbb{E}[\hat{Y}_n^{(t)} - Y_n^{(t)}] \rightarrow 1/2,
\end{align*}
with expectation taken over the data $\mathcal{D}_n^{(t)}$, as well as the randomness associated with model $f_n^{(t)}$.

We define the conditional density ratio at round $t$:
\begin{align*}
    r(\mathbf{x}, t) := \sum_{\ell: \mathbf{x} \in \mathcal{X}^\ell_t}  \frac{p(\tilde{\mathbf{x}}^{(t+1)} | \theta^\ell_t)}{p(\mathbf{x} | \theta^\ell_t)}. 
\end{align*}
Note that this value is well-defined for all $\mathbf{x}$, given the condition that $\mathbf{x} \in \mathcal{X}^\ell_t$. (The summation is effectively an indicator function over leaves.) As $n$ grows large, $r(\mathbf{x}, t)$ will converge on some constant $c \in \mathbb{R}_{\geq 0}$. Partition this range at $c=1$, creating $c_- \in [0,1)$ and $c_+ \in (1, \infty]$. Resulting behavior depends on whether $r(\mathbf{x}, t)$ converges to some value in the former or the latter range. (Of course, at $r(\mathbf{x}, t) = 1$, the optimum has been reached and no further rounds are required.) 

If $r(\mathbf{x}, t) \rightarrow c_-$, then $\mathcal{X}^\ell_t$ contains dependencies that were not well-modelled by the splits at round $t-1$. In the next round, synthetic data will be sampled from new splits that concentrate more closely on this neglected subregion, given its relatively high coverage. If $r(\mathbf{x}, t) \rightarrow c_+$, then $\mathcal{X}^\ell_t$ denotes a low-density region where synthetic data is more likely than true data. These leaves will be down-weighted in future rounds, as low-coverage regions are less likely to be selected for data generation.
Define the conditional entropy function at round $t$:
\begin{align*}
    H_t(Y|\mathbf{x}) := - \Big(f^{(t+1)}(\mathbf{x}) \log_2 f^{(t+1)}(\mathbf{x}) + \big(1 - f^{(t+1)}(\mathbf{x})\big) \log_2 \big(1 - f^{(t+1)}(\mathbf{x})\big) \Big).
\end{align*}

The honesty and regularity conditions originally introduced by \citet{Wager2018}---subsequently generalized by \citet{Athey2019} and further studied by \citet{Peng2022}---are well-suited to our task. They provide consistency criteria for regression forests that apply to RF classifiers as a special case when predictions are made via soft labeling. For full details, we refer readers to the original texts. 
We simply summarize the most pertinent result below, which is that RFs are asymptotically unbiased \citep[Thm.~3]{Wager2018}:
\begin{equation*}
    \big|\mathbb{E}[f(\mathbf{x})] - \mathbb{E}[Y|\mathbf{x}]\big| = \mathcal{O}\bigg( n_b^{- \frac{1}{2} \frac{\log( (1 - \gamma)^{-1})}{\log(\gamma^{-1})} \frac{\pi}{d} } \bigg).
\end{equation*}
Thus any RF classifier satisfying (A1)-(A3) will converge as $n$ grows large.\footnote{Strictly speaking, the honesty condition (ii) is not necessary to prove the consistency of RFs. However, it does tend to reduce bias, especially in the presence of outliers.  and, along with some further assumptions that we omit regarding subsampling rates, guarantees asymptotic normality of RF predictions. Alternative consistency conditions for adaptive split trees require either further assumptions about the data generating process \citep{Scornet2015} or modifications to the algorithm itself \citep{wager_walther}. See \citet[Appx.~B]{Wager2018} for a discussion.} 

Meanwhile, variance decays according to \citep[Appx.~C.2]{Wager2018}:
\begin{equation*}
    \mathbb{E}\bigg[ \Big[ f(\mathbf{x}) - \mathbb{E}[f(\mathbf{x})] \Big]^2 \bigg] = \mathcal{O}\bigg( n_b^{- \frac{\log( (1 - \gamma)^{-1})}{\log(\gamma^{-1})} \frac{\pi}{d} } \bigg).
\end{equation*}

\citet{biau_analysis} assumes that $\mathbb{E}[Y|\mathbf{x}]$ depends only on a subset of features $S \subset [d]$---a common occurrence in moderate to high dimensions, and something we empirically observed in several ARF experiments. Thus we should expect these so-called ``strong'' features to be selected with probability approaching $1/|S|$ as $n \rightarrow \infty$. Under these conditions, (A1)-(A3) imply the following \citep[Thm.~5]{biau_analysis}:
\begin{align*}
    \mathbb{E}\big[f(\mathbf{x}) - \mathbb{E}[Y|\mathbf{x}] \big]^2 = \mathcal{O}\big(n^{\frac{-0.75}{|S|\log2 + 0.75}}\big).
\end{align*}
Thus the convergence rate depends only on the number of strong features, rather than the ambient dimension $d$. 
\end{comment}






\subsection{Proof of Lemma~\ref{lm:decomp}} 
Define the first-order approximation to $p$ satisfying local independence:
\begin{equation*}\label{eq:fir}
    \hat{p}(\mathbf{x}) := \frac{1}{B} \sum_{\ell, b: \mathbf{x} \in \mathcal{X}^\ell_b} ~p(\theta_b^\ell) ~\prod_{j=1}^d p(x_j|\theta^\ell_b).
\end{equation*}
We also define the root integrated squared error (RISE), i.e. the Euclidean distance between probability densities:
\begin{equation*}
    \text{RISE}(p, q) := \bigg( \int_{\mathcal{X}} \Big( p(\mathbf{x}) - q(\mathbf{x}) \Big)^2 ~d\mathbf{x} \bigg)^{1/2}.
\end{equation*}
By the triangle inequality, we have:
\begin{align*}
    \text{RISE}(p, q) &\leq \text{RISE}(p, \hat{p}) + \text{RISE}(\hat{p}, q). 
\end{align*}
Squaring both sides, we get:
\begin{align*}
    \text{ISE}(p, q) &\leq \text{ISE}(p, \hat{p}) + \text{ISE}(\hat{p}, q) + 2  ~\text{RISE}(p, \hat{p}) ~\text{RISE}(\hat{p}, q). 
\end{align*}
Adding a nonnegative value to the rhs, we can reduce the expression:
\begin{align*}
    \text{ISE}(p, q) &\leq \text{ISE}(p, \hat{p}) + \text{ISE}(\hat{p}, q) + 2  ~\text{RISE}(p, \hat{p}) ~\text{RISE}(\hat{p}, q) + \big(\text{RISE}(p, \hat{p}) - \text{RISE}(\hat{p}, q) \big)^2 \\
    &= 2 \big( \text{ISE}(p, \hat{p}) + \text{ISE}(\hat{p}, q) \big).
\end{align*}
Now observe that we can rewrite both ISE formulae in terms of our predefined residuals (Eqs. \ref{eq:eps1}-\ref{eq:eps3}):
\begin{align*}
    \text{ISE}(p, \hat{p}) &= \int_\mathcal{X} \bigg(\frac{1}{B} \sum_{\ell, b: \mathbf{x} \in \mathcal{X}^\ell_b} \Big( p(\mathbf{x}|\theta^\ell_b)~p(\theta^\ell_b) - \prod_{j=1}^d p(x_j|\theta^\ell) ~p(\theta^\ell_b) \Big) \bigg)^2 ~d\mathbf{x} \\
    &= \frac{1}{B^2}\int_\mathcal{X} \bigg( \sum_{\ell, b: \mathbf{x} \in \mathcal{X}^\ell_b} p(\theta^\ell_b) \epsilon_3 \bigg)^2 ~d\mathbf{x}. \\
    \text{ISE}(\hat{p}, q) &= \int_\mathcal{X} \bigg(\frac{1}{B} \sum_{\ell, b: \mathbf{x} \in \mathcal{X}^\ell_b} \Big( \prod_{j=1}^d p(x_j|\theta^\ell_b) ~p(\theta^\ell_b) - \prod_{j=1}^d q(x_j; \bm{\theta}_{b,j}^\ell) ~q(\theta^\ell_b) \Big) \bigg)^2 ~d\mathbf{x} \\
    &= \frac{1}{B^2}\int_\mathcal{X} \bigg( \sum_{\ell, b: \mathbf{x} \in \mathcal{X}^\ell_b} \Big( p(\theta^\ell_b)\epsilon_2 + \epsilon_1\prod_{j=1}^d p(x_j|\theta^\ell_b) - \epsilon_1 \epsilon_2 \Big) \bigg)^2 ~d\mathbf{x}.
\end{align*}
We replace the interior squared terms for ease of presentation:
\begin{align*}
    \alpha &:= \sum_{\ell, b: \mathbf{x} \in \mathcal{X}_b^\ell} p(\theta^\ell_b) \epsilon_3 \\
    \beta &:= \sum_{\ell, b: \mathbf{x} \in \mathcal{X}_b^\ell} \Big( p(\theta^\ell_b)\epsilon_2 + \epsilon_1\prod_{j=1}^d p(x_j|\theta^\ell_b) - \epsilon_1 \epsilon_2 \Big).
\end{align*}
Finally, we take expectations on both sides:
\begin{align*}
    \text{MISE}(p, q) \leq 2B^{-2}~\mathbb{E} \Bigg[ \int_\mathcal{X} \alpha^2 + \beta^2 ~d\mathbf{x} \Bigg],
\end{align*}
where we have exploited the linearity of expectation to pull the factor outside of the bracketed term, and the monotonicity of expectation to preserve the inequality.

\subsection{Proof of Theorem~\ref{thm:cons}}\label{proof:l2}
Lemma~\ref{lm:decomp} states that error is bounded by a quadratic function of $\epsilon_1, \epsilon_2, \epsilon_3$. Thus for $L_2$-consistency, it suffices to show that $\mathbb{E}[\epsilon_j^2] \rightarrow 0$, for $j \in \{1, 2, 3\}$. Since this is already established by Thm.~\ref{thm:conv} for $j=3$, we focus here on errors of coverage and density. Start with $\epsilon_1$. A general version of the Glivenko-Cantelli theorem \citep{Vapnik2015} guarantees uniform convergence of empirical proportions to population proportions. Let $\mathcal{L}$ denote the set of all possible hyperrectangular subspaces induced by axis-aligned splits on $\mathcal{X}$. Then the following holds with probability 1: 
\begin{align*}
    \lim_{n \rightarrow \infty} \sup_{\ell \in \mathcal{L}} \big|p(\theta^\ell) - q_n(\theta^\ell)\big| = 0.
\end{align*}

Next, take $\epsilon_2$. (A4) guarantees that $p$ satisfies the consistency conditions for univariate KDE \citep{silverman1986, wand1994, Gramacki_kde}, while condition (v) of (A3) ensures that within-leaf sample size increases even as leaf volume goes to zero \citep[Lemma 2]{Meinshausen2006}. Our kernel is a nonnegative function $K: \mathbb{R}^d \rightarrow \mathbb{R}$ that integrates to 1, parametrized by the bandwidth $h$:
\begin{align*}
    p_h(\mathbf{x}) = \frac{1}{nh} \sum_{i=1}^n K\Big(\frac{\mathbf{x} - \mathbf{x}_i}{h}\Big).
\end{align*}
Using standard arguments, we take a Taylor series expansion of the MISE and minimize the \textit{asymptotic} MISE (AMISE):
\begin{equation*}
    \text{AMISE}(p, p_h) = \frac{1}{nh}R(K) + \frac{1}{4} h^4 \mu_2(K)^2R(p''),
\end{equation*}
where
\begin{align*}
    R(K) &= \int K(x)^2 ~dx, \\
    \mu_2(K) &= \int x^2 K(x) ~dx, ~\text{and}\\
    R(p'') &= \int p''(x)^2 ~dx.
\end{align*}
For example values of these variables under specific kernels, see \citep[Appx. B]{wand1994}. Under (A4), it can be shown that 
\begin{equation*}
    \text{MISE}(p, p_h) = \text{AMISE}(p, p_h) + o\big((nh)^{-1} + h^4\big).
\end{equation*}
Thus if $(nh)^{-1} \rightarrow 0$ and $h \rightarrow 0$ as $n \rightarrow \infty$, the asymptotic approximation is exact and $\mathbb{E}[\epsilon_2^2] \rightarrow 0$.  

These results, combined with the proof of Thm.~\ref{thm:conv} (see Appx.~\ref{proof:conv}), establish that errors of coverage, density, and convergence all vanish in the limit. Thus $\mathbb{E}[\epsilon_j^2] \rightarrow 0$ for $j \in \{1, 2, 3\}$, and the proof is complete.

\begin{comment}
Finally, take $\epsilon_3$. The expected square of this value goes to zero if and only if the joint distribution of predictors within each leaf factorizes as a product of marginals, in which case our ARF has converged. Thus our goal in this section is to prove the consistency of this algorithm. First, we consider the criterion that conditional entropy $H(Y|\theta^\ell_b) = 1$ for all $\ell, b$. If this does not hold as depth increases, then Alg.~\ref{alg:garf} will fail to terminate. Given our recursive split-and-resample strategy, such a failure can only occur if the distribution is self-similar, with dependencies replicating at ever finer resolutions as in some fractal equations \citep{mandelbrot1982}. Yet such functions are nowhere differentiable, as originally demonstrated by Weierstrass \citep{Weierstrass1895}. Rademacher's theorem states that Lipschitz continuous functions are differentiable almost everywhere, and thus (A2) rules out such pathological cases.
\end{comment}








==> AISTATS/kde.tex <==
We can in principle use random forests for kernel density estimation (KDE). The basic formula for KDE is:
\begin{equation}
    \hat{f}(\mathbf{x}) = \frac{1}{n} \sum_{i=1}^n k(\mathbf{x}, \mathbf{x}_i),
\end{equation}
where $\hat{f}$ is an estimate of the true density function $f$, and $k: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}_+$ is a kernel that measures some notion of distance in $P_X$. Recall that random forests effectively learn an adaptive kernel on $[0,1]$, representing the proportion of leaves in which two samples co-occur. This amounts to an efficient and adaptive density estimator, with several advantages: (a) completely nonparametric and likelihood-free; (b) works with mixed data; (c) performs automatic feature selection; (d) fast. I would use unsupervised RF as the basis learner so we're not optimized for some particular outcome, but rather focus on internal dependencies between predictors. Then we have:
\begin{equation}
    k(\mathbf{x}, \mathbf{x}') = 1 - \frac{\#\{l: \phi_l \vDash \mathbf{x}, \mathbf{x}'\}}{|L|}.
\end{equation}

Idea: is there some way to exploit "proximity to a leaf"? It may be true that each point only falls into one leaf, but there is a partial ordering on leaves representing how close it comes to satisfying the conjunction of split criteria for each. Also, earlier splits should be weighed more heavily. Would this give more information?

Idea: impose conditional independence constraints via restrictions on variable splits. To split in an RF is to condition. To find the best approximation to $X \leftarrow Z \rightarrow Y$ (with no further dependencies), we impose a rule that trees can split on any two of these features but never all three. Question: is there some simple set of rules for translating DAGs into such splitting restrictions? I'm sure there is. 

==> kde.tex <==
We can in principle use random forests for kernel density estimation (KDE). The basic formula for KDE is:
\begin{equation}
    \hat{f}(\mathbf{x}) = \frac{1}{n} \sum_{i=1}^n k(\mathbf{x}, \mathbf{x}_i),
\end{equation}
where $\hat{f}$ is an estimate of the true density function $f$, and $k: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}_+$ is a kernel that measures some notion of distance in $P_X$. Recall that random forests effectively learn an adaptive kernel on $[0,1]$, representing the proportion of leaves in which two samples co-occur. This amounts to an efficient and adaptive density estimator, with several advantages: (a) completely nonparametric and likelihood-free; (b) works with mixed data; (c) performs automatic feature selection; (d) fast. I would use unsupervised RF as the basis learner so we're not optimized for some particular outcome, but rather focus on internal dependencies between predictors. Then we have:
\begin{equation}
    k(\mathbf{x}, \mathbf{x}') = 1 - \frac{\#\{l: \phi_l \vDash \mathbf{x}, \mathbf{x}'\}}{|L|}.
\end{equation}

Idea: is there some way to exploit "proximity to a leaf"? It may be true that each point only falls into one leaf, but there is a partial ordering on leaves representing how close it comes to satisfying the conjunction of split criteria for each. Also, earlier splits should be weighed more heavily. Would this give more information?

Idea: impose conditional independence constraints via restrictions on variable splits. To split in an RF is to condition. To find the best approximation to $X \leftarrow Z \rightarrow Y$ (with no further dependencies), we impose a rule that trees can split on any two of these features but never all three. Question: is there some simple set of rules for translating DAGs into such splitting restrictions? I'm sure there is. 
